Bottomonia in quark-antiquark confining potential

In this paper, we comprehensively explore bottomonia mass spectra and their decay properties by solving the non-relativistic Schrodinger wave equation numerically with approximate quark-antiquark potential form. We also incorporate spin-dependent terms - spin-spin, spin-orbit, and tensor terms to remove mass degeneracy and to obtain excited states ($nS, nP, nD, nF, n = 1, 2, 3, 4, 5$) mass spectra. By using Van Royen - Weisskopf formula, we investigate leptonic decay constants, di-leptonic, di-gamma, tri-gamma, di-gluon decay widths and also incorporate first-order radiative corrections. We also computed radiative transition widths, which give a better insight into the non-perturbative aspects of QCD. The present results for mass spectroscopy and decay properties are in tune with available experimental values and other theoretical predictions. Our results may provide better insight to upcoming experimental information in the near future.

==> bbl <==
\begin{thebibliography}{82}

\bibitem{herb1977}
S.W. Herb, D.C. Hom, L.M. Lederman, J.C. Sens, H.D. Snyder, J.K. Yoh, J.A.
  Appel, B.C. Brown, C.N. Brown, W.R. Innes et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.39.252}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.39.252}{39}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.39.252}{252}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.39.252}{1977})

\bibitem{Innes1977}
W.R. Innes, J.A. Appel, B.C. Brown, C.N. Brown, K.~Ueno, T.~Yamanouchi, S.W.
  Herb, D.C. Hom, L.M. Lederman, J.C. Sens et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.39.1240}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.39.1240}{39}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.39.1240}{1240}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.39.1240}{1977})

\bibitem{PDG2022}
R.L. Workman, Others (Particle Data Group),
  \href{https://doi.org/10.1093/ptep/ptac097}{PTEP}
  \textbf{\href{https://doi.org/10.1093/ptep/ptac097}{2022}},
  \href{https://doi.org/10.1093/ptep/ptac097}{083C01}
  (\href{https://doi.org/10.1093/ptep/ptac097} {2022})

\bibitem{han1982}
K.~Han, T.~B\"ohringer, P.~Franzini, G.~Mageras, D.~Peterson, E.~Rice, J.K.
  Yoh, J.E. Horstkotte, C.~Klopfenstein, J.~Lee-Franzini et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1612}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1612}{49}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1612}{1612}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1612}{1982})

\bibitem{eigen1982}
G.~Eigen, G.~Blanar, H.~Dietl, E.~Lorenz, F.~Pauss, H.~Vogel, T.~B\"ohringer,
  P.~Franzini, K.~Han, G.~Mageras et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1616}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1616}{49}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1616}{1616}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.49.1616}{1982})

\bibitem{klopfenstein1983}
C.~Klopfenstein, J.E. Horstkotte, J.~Lee-Franzini, R.D. Schamberger,
  M.~Sivertz, L.J. Spencer, P.M. Tuts, P.~Franzini, K.~Han, E.~Rice et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.51.160}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.51.160}{51}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.51.160}{160}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.51.160}{1983})

\bibitem{fpauss1983}
F.~Pauss, H.~Dietl, G.~Eigen, E.~Lorenz, G.~Mageras, H.~Vogel, P.~Franzini,
  K.~Han, D.~Peterson, E.~Rice et~al.,
  \href{https://doi.org/10.1016/0370-2693(83)91539-3}{Physics Letters B}
  \textbf{\href{https://doi.org/10.1016/0370-2693(83)91539-3}{130}}, {439}
  (\href{https://doi.org/10.1016/0370-2693(83)91539-3}{1983})

\bibitem{besson1985}
D.~Besson, J.~Green, R.~Namjoshi, F.~Sannes, P.~Skubic, A.~Snyder, R.~Stone,
  A.~Chen, M.~Goldberg, N.~Horwitz et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.54.381}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.54.381}{54}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.54.381}{381}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.54.381}{1985})

\bibitem{lovelock1985}
D.M.J. Lovelock, J.E. Horstkotte, C.~Klopfenstein, J.~Lee-Franzini, L.~Romero,
  R.D. Schamberger, S.~Youssef, P.~Franzini, D.~Son, P.M. Tuts et~al.,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.54.377}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.54.377}{54}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.54.377}{377}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.54.377}{1985})

\bibitem{aubert2008}
B.~Aubert, M.~Bona, Y.~Karyotakis, J.P. Lees, V.~Poireau, E.~Prencipe,
  X.~Prudent, V.~Tisserand, J.~Garra~Tico, E.~Grauges et~al. (BABAR
  Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.101.071801}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.101.071801}{101}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.101.071801}{071801}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.101.071801}{2008})

\bibitem{del2010}
P.~del Amo~Sanchez, J.P. Lees, V.~Poireau, E.~Prencipe, V.~Tisserand,
  J.~Garra~Tico, E.~Grauges, M.~Martinelli, A.~Palano, M.~Pappagallo et~al.
  ({BABAR Collaboration}),
  \href{https://link.aps.org/doi/10.1103/PhysRevD.82.111102}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.82.111102}{82}},
  \href{https://link.aps.org/doi/10.1103/PhysRevD.82.111102}{111102}
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.82.111102}{2010})

\bibitem{lees2011}
J.P. Lees, V.~Poireau, E.~Prencipe, V.~Tisserand, J.~Garra~Tico, E.~Grauges,
  M.~Martinelli, D.A. Milanes, A.~Palano, M.~Pappagallo et~al. (The BABAR
  Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevD.84.091101}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.84.091101}{84}},
  \href{https://link.aps.org/doi/10.1103/PhysRevD.84.091101}{091101}
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.84.091101}{2011})

\bibitem{adachi2012}
I.~Adachi, H.~Aihara, K.~Arinstein, D.M. Asner, T.~Aushev, T.~Aziz, A.M.
  Bakich, E.~Barberio, K.~Belous, V.~Bhardwaj et~al. (Belle Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.108.032001}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.108.032001}{108}},
  032001 (\href{https://link.aps.org/doi/10.1103/PhysRevLett.108.032001}{2012})

\bibitem{aad2012}
G.~Aad, B.~Abbott, J.~Abdallah, A.A. Abdelalim, A.~Abdesselam, O.~Abdinov,
  B.~Abi, M.~Abolins, O.S. AbouZeid, H.~Abramowicz et~al. (ATLAS
  Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.108.152001}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.108.152001}{108}},
  152001 (\href{https://link.aps.org/doi/10.1103/PhysRevLett.108.152001}{2012})

\bibitem{abazov2012}
V.M. Abazov, B.~Abbott, B.S. Acharya, M.~Adams, T.~Adams, G.D. Alexeev,
  G.~Alkhazov, A.~Alton, G.~Alverson, M.~Aoki et~al. (D0 Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevD.86.031103}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.86.031103}{86}},
  031103 (\href{https://link.aps.org/doi/10.1103/PhysRevD.86.031103}{2012})

\bibitem{aaij2014}
R.~Aaij, , B.~Adeva, M.~Adinolfi, A.~Affolder, Z.~Ajaltouni, S.~Akar,
  J.~Albrecht, F.~Alessio, M.~Alexander et~al.,
  \href{https://doi.org/10.1007%2Fjhep10%282014%29088}{Journal of High Energy
  Physics} \textbf{{2014}}, 088
  (\href{https://doi.org/10.1007%2Fjhep10%282014%29088}{2014})

\bibitem{sirunyan2018}
A.M. Sirunyan, A.~Tumasyan, W.~Adam, F.~Ambrogi, E.~Asilar, T.~Bergauer,
  J.~Brandstetter, M.~Dragicevic, J.~Er\"o, A.~Escalante Del~Valle et~al. (CMS
  Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.120.231801}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.120.231801}{120}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.120.231801}{231801}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.120.231801}{2018})

\bibitem{mizuk2012}
R.~Mizuk, D.M. Asner, A.~Bondar, T.K. Pedlar, I.~Adachi, H.~Aihara,
  K.~Arinstein, V.~Aulchenko, T.~Aushev, T.~Aziz et~al. (Belle Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.109.232002}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.109.232002}{109}},
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.109.232002}{232002}
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.109.232002}{2012})

\bibitem{wu2020}
Q.~Wu, D.Y. Chen, T.~Matsuki,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.102.114037}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.102.114037}{102}},
  \href{https://link.aps.org/doi/10.1103/PhysRevD.102.114037}{114037}
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.102.114037}{2020})

\bibitem{wang2014}
Z.G. Wang, T.~Huang,
  \href{https://doi.org/10.1016/j.nuclphysa.2014.08.084}{Nucl. Phys. A}
  \textbf{\href{https://doi.org/10.1016/j.nuclphysa.2014.08.084}{930}},
  \href{https://doi.org/10.1016/j.nuclphysa.2014.08.084}{63}
  (\href{https://doi.org/10.1016/j.nuclphysa.2014.08.084}{2014})

\bibitem{chen2014}
D.Y. Chen, X.~Liu, T.~Matsuki,
  \href{https://iopscience.iop.org/article/10.1088/1674-1137/38/5/053102}{Chin.
  Phys. C}
  \textbf{\href{https://iopscience.iop.org/article/10.1088/1674-1137/38/5/053102}{38}},
  {053102}
  (\href{https://iopscience.iop.org/article/10.1088/1674-1137/38/5/053102}{2014})

\bibitem{mizuk2019}
R.~Mizuk, A.~Bondar, I.~Adachi, H.~Aihara, D.~Asner, V.~Aulchenko, T.~Aushev,
  R.~Ayad, I.~Badhrees, S.~Bahinipati et~al., Journal of High Energy Physics
  \textbf{2019} (2019), cited by: 33; All Open Access, Gold Open Access, Green
  Open Access

\bibitem{chen2020}
B.~Chen, A.~Zhang, J.~He,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.101.014020}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.101.014020}{101}},
  \href{https://link.aps.org/doi/10.1103/PhysRevD.101.014020}{014020}
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.101.014020}{2020})

\bibitem{wang2019}
Z.G. Wang,
  \href{http://cpc.ihep.ac.cn/article/doi/10.1088/1674-1137/43/12/123102}{Chin.
  Phys. C}
  \textbf{\href{http://cpc.ihep.ac.cn/article/doi/10.1088/1674-1137/43/12/123102}{43}},
  {123102}
  (\href{http://cpc.ihep.ac.cn/article/doi/10.1088/1674-1137/43/12/123102}{2019}),
  \texttt{1905.06610}

\bibitem{deng2017}
W.J. Deng, H.~Liu, L.C. Gui, X.H. Zhong,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.95.074002}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.95.074002}{95}},
  {074002} (\href{https://link.aps.org/doi/10.1103/PhysRevD.95.074002}{2017})

\bibitem{wang2018}
J.Z. Wang, Z.F. Sun, X.~Liu, T.~Matsuki,
  \href{https://link.springer.com/article/10.1140/epjc/s10052-018-6372-1}{Eur.
  Phys. J. C}
  \textbf{\href{https://link.springer.com/article/10.1140/epjc/s10052-018-6372-1}{78}},
  {915}
  (\href{https://link.springer.com/article/10.1140/epjc/s10052-018-6372-1}{2018}),
  \texttt{1802.04938}

\bibitem{pandya2021}
B.~Pandya, M.~Shah, P.C. Vinodkumar,
  \href{https://link.springer.com/article/10.1140/epjc/s10052-021-08901-7}{Eur.
  Phys. J. C}
  \textbf{\href{https://link.springer.com/article/10.1140/epjc/s10052-021-08901-7}{81}},
  {116}
  (\href{https://link.springer.com/article/10.1140/epjc/s10052-021-08901-7}{2021})

\bibitem{chaturvedi2020}
R.~Chaturvedi, A.K. Rai, N.R. Soni, J.N. Pandya,
  \href{https://dx.doi.org/10.1088/1361-6471/abaa99}{Journal of Physics G:
  Nuclear and Particle Physics}
  \textbf{\href{https://dx.doi.org/10.1088/1361-6471/abaa99}{47}}, {115003}
  (\href{https://dx.doi.org/10.1088/1361-6471/abaa99}{2020})

\bibitem{adachi2023}
I.~Adachi, L.~Aggarwal, H.~Ahmed, H.~Aihara, N.~Akopov, A.~Aloisio, N.~Anh~Ky,
  D.M. Asner, T.~Aushev, V.~Aushev et~al. (Belle II Collaboration),
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.130.091902}{Phys. Rev.
  Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.130.091902}{130}},
  091902 (\href{https://link.aps.org/doi/10.1103/PhysRevLett.130.091902}{2023})

\bibitem{eichten1980}
E.~Eichten, K.~Gottfried, T.~Kinoshita, K.D. Lane, T.M. Yan,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.21.203}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.21.203}{21}}, 203
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.21.203}{1980})

\bibitem{nrsoni2018}
N.R. Soni, B.R. Joshi, R.P. Shah, H.R. Chauhan, J.N. Pandya, Eur. Phys. J. C
  \textbf{78}, 592 (2018), \texttt{1707.07144}

\bibitem{kher2022}
V.~Kher, R.~Chaturvedi, N.~Devlani, A.K. Rai,
  \href{https://link.springer.com/article/10.1140/epjp/s13360-022-02538-5}{Eur.
  Phys. J. Plus}
  \textbf{\href{https://link.springer.com/article/10.1140/epjp/s13360-022-02538-5}{137}},
  357
  (\href{https://link.springer.com/article/10.1140/epjp/s13360-022-02538-5}{2022})

\bibitem{martin1980}
A.~Martin,
  \href{https://www.sciencedirect.com/science/article/pii/0370269380905274}{Physics
  Letters B}
  \textbf{\href{https://www.sciencedirect.com/science/article/pii/0370269380905274}{93}},
  {338}
  (\href{https://www.sciencedirect.com/science/article/pii/0370269380905274}{1980})

\bibitem{jena1983}
S.~Jena, T.~Tripati,
  \href{https://www.sciencedirect.com/science/article/pii/0370269383907888}{Physics
  Letters B}
  \textbf{\href{https://www.sciencedirect.com/science/article/pii/0370269383907888}{122}},
  {181
  (\href{https://www.sciencedirect.com/science/article/pii/0370269383907888}{1983})

\bibitem{quigg1977}
C.~Quigg, J.L. Rosner,
  \href{https://www.sciencedirect.com/science/article/pii/0370269377907651}{Physics
  Letters B}
  \textbf{\href{https://www.sciencedirect.com/science/article/pii/0370269377907651}{71}},
  153
  (\href{https://www.sciencedirect.com/science/article/pii/0370269377907651}{1977})

\bibitem{richardson1979}
J.L. Richardson,
  \href{https://www.sciencedirect.com/science/article/pii/0370269379907536}{Physics
  Letters B}
  \textbf{\href{https://www.sciencedirect.com/science/article/pii/0370269379907536}{82}},
  272
  (\href{https://www.sciencedirect.com/science/article/pii/0370269379907536}{1979})

\bibitem{song1987}
X.t. Song, H.f. Lin,
  \href{https://link.springer.com/article/10.1007/BF01566763}{Z. Phys. C}
  \textbf{\href{https://link.springer.com/article/10.1007/BF01566763}{34}}, 223
  (\href{https://link.springer.com/article/10.1007/BF01566763}{1987})

\bibitem{smruti2016}
S.~Patel, P.C. Vinodkumar, S.~Bhatnagar,
  \href{https://iopscience.iop.org/article/10.1088/1674-1137/40/5/053102}{Chin.
  Phys. C}
  \textbf{\href{https://iopscience.iop.org/article/10.1088/1674-1137/40/5/053102}{40}},
  053102
  (\href{https://iopscience.iop.org/article/10.1088/1674-1137/40/5/053102}{2016})

\bibitem{mittal1986}
A.~Mittal, A.N. Mitra, Phys. Rev. Lett. \textbf{57}, 290 (1986)

\bibitem{gupta1990}
K.K. Gupta, A.N. Mitra, N.N. Singh, Phys. Rev. D \textbf{42}, 1604 (1990)

\bibitem{sharma1994}
A.~Sharma, S.R. Choudhury, A.N. Mitra, Phys. Rev. D \textbf{50}, 454 (1994)

\bibitem{Nsingh1988}
N.N. Singh, A.N. Mitra,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.38.1454}{Phys. Rev. D}
  \textbf{{38}}, 1454
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.38.1454}{1988})

\bibitem{CHAKRABARTY1989}
S.~Chakrabarty, K.~Gupta, N.~Singh, A.~Mitra,
  \href{https://doi.org/10.1016/0146-6410(89)90003-3}{Progress in Particle and
  Nuclear Physics}
  \textbf{\href{https://doi.org/10.1016/0146-6410(89)90003-3}{22}}, 43
  (\href{https://doi.org/10.1016/0146-6410(89)90003-3}{1989})

\bibitem{anumittal1986}
A.~Mittal, A.N. Mitra,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.57.290}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.57.290}{57}}, 290
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.57.290}{1986})

\bibitem{kkgupta1990}
K.K. Gupta, A.N. Mitra, N.N. Singh,
  {https://link.aps.org/doi/10.1103/PhysRevD.42.1604}{Phys. Rev. D}
  \textbf{{https://link.aps.org/doi/10.1103/PhysRevD.42.1604}{42}}, 1604
  ({https://link.aps.org/doi/10.1103/PhysRevD.42.1604}{1990})

\bibitem{asharma1994}
A.~Sharma, S.R. Choudhury, A.N. Mitra,
  {https://link.aps.org/doi/10.1103/PhysRevD.50.454}{Phys. Rev. D}
  \textbf{{https://link.aps.org/doi/10.1103/PhysRevD.50.454}{50}}, 454
  ({https://link.aps.org/doi/10.1103/PhysRevD.50.454}{1994})

\bibitem{ALKOFER2001}
R.~Alkofer, L.~{von Smekal},
  \href{https://doi.org/10.1016/S0370-1573(01)00010-2}{Physics Reports}
  \textbf{\href{https://doi.org/10.1016/S0370-1573(01)00010-2}{353}}, 281
  (\href{https://doi.org/10.1016/S0370-1573(01)00010-2}{2001})

\bibitem{alkofer2002}
R.~Alkofer, P.~Watson, H.~Weigel,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.65.094026}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.65.094026}{65}},
  094026 (\href{https://link.aps.org/doi/10.1103/PhysRevD.65.094026}{2002})

\bibitem{CVETIC2004}
G.~Cvetič, C.~Kim, G.L. Wang, W.~Namgung,
  \href{https://doi.org/10.1016/j.physletb.2004.06.092}{Physics Letters B}
  \textbf{\href{https://doi.org/10.1016/j.physletb.2004.06.092}{596}}, 84
  (\href{https://doi.org/10.1016/j.physletb.2004.06.092}{2004})

\bibitem{Bhatnagar_2006}
S.~Bhatnagar, S.Y. Li,
  \href{https://dx.doi.org/10.1088/0954-3899/32/7/005}{Journal of Physics G:
  Nuclear and Particle Physics}
  \textbf{\href{https://dx.doi.org/10.1088/0954-3899/32/7/005}{32}}, 949
  (\href{https://dx.doi.org/10.1088/0954-3899/32/7/005}{2006})

\bibitem{bhatnagar2014}
S.~Bhatnagar, J.~Mahecha, Y.~Mengesha,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.90.014034}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.90.014034}{90}},
  014034 (\href{https://link.aps.org/doi/10.1103/PhysRevD.90.014034}{2014})

\bibitem{voloshin2008}
M.~Voloshin,
  \href{https://www.sciencedirect.com/science/article/pii/S0146641008000239}{Progress
  in Particle and Nuclear Physics}
  \textbf{\href{https://www.sciencedirect.com/science/article/pii/S0146641008000239}{61}},
  455
  (\href{https://www.sciencedirect.com/science/article/pii/S0146641008000239}{2008})

\bibitem{berestetskii1982}
V.~Berestetskii, E.~Lifshits, L.~Pitaevskii,
  \emph{\href{https://shop.elsevier.com/books/quantum-electrodynamics/berestetskii/978-0-08-050346-2}{Quantum
  Electrodynamics}} (Pergamon, 1982)

\bibitem{gershtein1995}
S.S. Gershtein, V.V. Kiselev, A.K. Likhoded, A.V. Tkabladze,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.51.3613}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.51.3613}{51}}, {3613}
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.51.3613}{1995})

\bibitem{lucha1999}
W.~Lucha, F.F. Schoberl,
  \href{https://www.worldscientific.com/doi/abs/10.1142/S0129183199000450}{Int.
  J. Mod. Phys. C}
  \textbf{\href{https://www.worldscientific.com/doi/abs/10.1142/S0129183199000450}{10}},
  607
  (\href{https://www.worldscientific.com/doi/abs/10.1142/S0129183199000450}{1999})

\bibitem{godfrey2015}
S.~Godfrey, K.~Moats,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.92.054034}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.92.054034}{92}},
  054034 (\href{https://link.aps.org/doi/10.1103/PhysRevD.92.054034}{2015})

\bibitem{shah2012}
M.~Shah, A.~Parmar, P.C. Vinodkumar,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.86.034015}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.86.034015}{86}},
  034015 (\href{https://link.aps.org/doi/10.1103/PhysRevD.86.034015}{2012})

\bibitem{ebert2011}
D.~Ebert, R.N. Faustov, V.O. Galkin, Eur. Phys. J. C \textbf{71}, 1825 (2011),
  \texttt{1111.0454}

\bibitem{radford2011}
S.F. Radford, W.W. Repko, Nucl. Phys. A \textbf{865}, 69 (2011),
  \texttt{0912.2259}

\bibitem{godfrey1985}
S.~Godfrey, N.~Isgur,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.32.189}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.32.189}{32}}, 189
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.32.189}{1985})

\bibitem{li2009}
B.Q. Li, K.T. Chao, Commun. Theor. Phys. \textbf{52}, 653 (2009),
  \texttt{0909.1369}

\bibitem{van1967}
R.~Van~Royen, V.F. Weisskopf,
  \href{https://link.springer.com/article/10.1007/BF02823542}{Nuovo Cim. A}
  \textbf{\href{https://link.springer.com/article/10.1007/BF02823542}{50}},
  {617} (\href{https://link.springer.com/article/10.1007/BF02823542}{1967}),
  \href{http://dx.doi.org/10.1007/BF02902203}{[Erratum: Nuovo Cim.A 51, 583
  (1967)]}

\bibitem{braaten1995}
E.~Braaten, S.~Fleming,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.52.181}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.52.181}{52}}, 181
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.52.181}{1995})

\bibitem{berezhnoy1996}
A.V. Berezhnoy, V.V. Kiselev, A.K. Likhoded,
  \href{https://link.springer.com/article/10.1007/s002180050152}{Z. Phys. A}
  \textbf{\href{https://link.springer.com/article/10.1007/s002180050152}{356}},
  89 (\href{https://link.springer.com/article/10.1007/s002180050152}{1996})

\bibitem{eichten1975}
E.~Eichten, K.~Gottfried, T.~Kinoshita, J.~Kogut, K.D. Lane, T.M. Yan,
  \href{https://link.aps.org/doi/10.1103/PhysRevLett.34.369}{Phys. Rev. Lett.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevLett.34.369}{34}}, 369
  (\href{https://link.aps.org/doi/10.1103/PhysRevLett.34.369}{1975})

\bibitem{eichten1978}
E.~Eichten, K.~Gottfried, T.~Kinoshita, K.D. Lane, T.M. Yan,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.17.3090}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.17.3090}{17}}, 3090
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.17.3090}{1978})

\bibitem{brambilla2006}
N.~Brambilla, Y.~Jia, A.~Vairo,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.73.054005}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.73.054005}{73}},
  054005 (\href{https://link.aps.org/doi/10.1103/PhysRevD.73.054005}{2006})

\bibitem{li2011}
D.M. Li, P.F. Ji, B.~Ma,
  \href{https://link.springer.com/article/10.1140/epjc/s10052-011-1582-9}{Eur.
  Phys. J. C}
  \textbf{\href{https://link.springer.com/article/10.1140/epjc/s10052-011-1582-9}{71}},
  1582
  (\href{https://link.springer.com/article/10.1140/epjc/s10052-011-1582-9}{2011})

\bibitem{kwong1988}
W.~Kwong, P.B. Mackenzie, R.~Rosenfeld, J.L. Rosner,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.37.3210}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.37.3210}{37}}, 3210
  (\href{https://link.aps.org/doi/10.1103/PhysRevD.37.3210}{1988})

\bibitem{landu1948}
L.D. Landau,
  \href{https://www.sciencedirect.com/science/article/abs/pii/B9780080105864500705?via%3Dihub}{Dokl.
  Akad. Nauk SSSR} \textbf{{60}}, 207
  (\href{https://www.sciencedirect.com/science/article/abs/pii/B9780080105864500705?via%3Dihub}{1948})

\bibitem{yang1950}
C.N. Yang, \href{https://link.aps.org/doi/10.1103/PhysRev.77.242}{Phys. Rev.}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRev.77.242}{77}}, 242
  (\href{https://link.aps.org/doi/10.1103/PhysRev.77.242}{1950})

\bibitem{lansberg2009}
J.P. Lansberg, T.N. Pham,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.79.094016}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.79.094016}{79}},
  094016 (\href{https://link.aps.org/doi/10.1103/PhysRevD.79.094016}{2009})

\bibitem{barbieri1981}
R.~Barbieri, M.~Caffo, R.~Gatto, E.~Remiddi,
  \href{https://www.sciencedirect.com/science/article/abs/pii/0550321381901929?via%3Dihub}{Nucl.
  Phys. B} \textbf{{192}}, 61
  (\href{https://www.sciencedirect.com/science/article/abs/pii/0550321381901929?via%3Dihub}{1981})

\bibitem{mangano1995}
M.L. Mangano, A.~Petrelli,
  \href{https://www.sciencedirect.com/science/article/pii/037026939500516N?via%3Dihub}{Phys.
  Lett. B} \textbf{{352}}, 445
  (\href{https://www.sciencedirect.com/science/article/pii/037026939500516N?via%3Dihub}{1995}),
  \texttt{hep-ph/9503465}

\bibitem{krassnigg2016}
A.~Krassnigg, M.~Gomez-Rocha, T.~Hilger, J. Phys. Conf. Ser. \textbf{742},
  012032 (2016), \texttt{1603.07232}

\bibitem{patel2009}
B.~Patel, P.C. Vinodkumar, J. Phys. G \textbf{36}, 035003 (2009),
  \texttt{0808.2888}

\bibitem{wang2006}
G.L. Wang, Phys. Lett. B \textbf{633}, 492 (2006), \texttt{math-ph/0512009}

\bibitem{bhavsar2018}
T.~Bhavsar, M.~Shah, P.C. Vinodkumar, Eur. Phys. J. C \textbf{78}, 227 (2018),
  \texttt{1803.07249}

\bibitem{radford2007}
S.F. Radford, W.W. Repko, Phys. Rev. D \textbf{75}, 074031 (2007)

\bibitem{ebert2003}
D.~Ebert, R.N. Faustov, V.O. Galkin, Phys. Rev. D \textbf{67}, 014027 (2003),
  \texttt{hep-ph/0210381}

\bibitem{bhaghyesh2011}
Bhaghyesh, K.B.V. Kumar, A.P. Monteiro, Journal of Physics G: Nuclear and
  Particle Physics \textbf{38}, 085001 (2011)

\bibitem{segovia2016}
J.~Segovia, P.G. Ortega, D.R. Entem, F.~Fern\'andez,
  \href{https://link.aps.org/doi/10.1103/PhysRevD.93.074027}{Phys. Rev. D}
  \textbf{\href{https://link.aps.org/doi/10.1103/PhysRevD.93.074027}{93}},
  074027 (\href{https://link.aps.org/doi/10.1103/PhysRevD.93.074027}{2016})

\end{thebibliography}

